A biologically plausible neural network for local supervision in cortical microcircuits

The backpropagation algorithm is an invaluable tool for training artificial neural networks; however, because of a weight sharing requirement, it does not provide a plausible model of brain function. Here, in the context of a two-layer network, we derive an algorithm for training a neural network which avoids this problem by not requiring explicit error computation and backpropagation. Furthermore, our algorithm maps onto a neural network that bears a remarkable resemblance to the connectivity structure and learning rules of the cortex. We find that our algorithm empirically performs comparably to backprop on a number of datasets.

==> old-stuff/old-figures/cca_circuit.tex <==
\begin{tikzpicture}
    %x inputs
    \coordinate (a1) at (0,0);
    \coordinate[right=6.4cm of a1] (a1R);
    \path[-, thick,  black!10!red] (a1) edge (a1R);
    \coordinate[above=.2cm of a1] (a2);
    \coordinate[right=6.4cm of a2] (a2R);
    \path[-, thick,  black!10!red] (a2) edge (a2R);
    \node[ainput] at ($(a1)!0.5!(a2)$) {${\y}$};

    %pyramidal neurons
    \node[zneuron, below right=1.9cm and 1.2cm of a1] (z1) {};
    \node at (z1) {$z_1$};
    \node[zneuron, right=2.2cm of z1] (zd) {};
    \node at (zd) {$z_k$};
    \node at ([yshift=-0cm]$(z1)!0.5!(zd)$) (zdots) {$\cdots$};
    \node[apical, above=2.2cm of z1] (z1A) {};
    \node[apical, above=2.2cm of zd] (zdA) {};
    
    \path[thick] (z1) edge (z1A);
    \path[thick] (zd) edge (zdA);
    
    %y inputs
    \coordinate[below=2.9cm of a1] (b1);
    \coordinate[right=6.4cm of b1] (b1R);
    \path[-, white!10!blue, thick] (b1) edge (b1R);
    \coordinate[below=.2cm of b1] (b2);
    \coordinate[right=6.4cm of b2] (b2R);
    \path[-, white!10!blue, thick] (b2) edge (b2R);
    \coordinate[below=.2cm of b2] (b3);
    \coordinate[right=6.4cm of b3] (b3R);
    \path[-, white!10!blue, thick] (b3) edge (b3R);
    \node[binput] at (b2) {${\x}$};

    %interneuron
    \coordinate[below left=-2.0cm and 0.75cm of b1R] (i1);
    \coordinate[left=5.95cm of i1] (i1R);
    \coordinate[above right=.2cm and .2cm of i1] (i2);
    \coordinate[above=.2cm of i1R] (i2R);
    % \coordinate[below right=.2cm and .2cm of i2] (i3);
    % \coordinate[below=.2cm of i2R] (i3R);

    \coordinate[below=3.3cm of i1] (int1N);
    \coordinate[right=.2cm of int1N] (int2N);
    % \coordinate[right=.2cm of int2N] (int3N);
    % \node[ineuron] at (int3N) (int3) {};
    \node[ineuron] at (int2N) (int2) {};
    \node[ineuron] at (int1N) (int1) {$\n$};
    
    \draw[-stealth,  black!30!green, thick] (int1) -- (i1) -- (i1R);
    \draw[-stealth,  black!30!green, thick] (int2) -- (i2) -- (i2R);
    % \draw[-stealth,  black!30!green, thick] (int3) -- (i3) -- (i3R);

    %apical synapses
    %\node[above left=1cm and .3cm of z1A] (z1A1) {};
    %\path[-, thick] (z1A) edge (z1A1);
    %\node[above right=1cm and .3cm of z1A] (z1A2) {};
    %\path[-, thick] (z1A) edge (z1A2);
    \node[asynapse] at (intersection of z1--z1A and a2--a2R) {};
    \node[asynapse] at (intersection of z1--z1A and a1--a1R) (as1) {};
    % \node[below left=-.01cm and -.1cm of as1] {${\color{red}a_1}$};

    %\node[above left=1cm and .3cm of zdA] (zdA1) {};
    %\path[-, thick] (zdA) edge (zdA1);
    %\node[above right=1cm and .3cm of zdA] (zdA2) {};
    %\path[-, thick] (zdA) edge (zdA2);
    \node[asynapse] at (intersection of zd--zdA and a2--a2R) {};
    \node[asynapse] at (intersection of zd--zdA and a1--a1R) (asd) {};
    % \node[below left=-.01cm and -.1cm of asd] {${\color{red}a_k}$};

    %axon
    \coordinate[below=2.45cm of z1] (z1Axon) {};
    \coordinate[below=2.25cm of zd] (zdAxon) {};

    \coordinate[right=4.85cm of z1Axon] (pyA1);
    \coordinate[above=.2cm of pyA1] (pyA2);
    
    \draw[-stealth, very thick] (z1) -- (z1Axon) -- (pyA1);
    \draw[-stealth, very thick] (zd) -- (zdAxon) -- (pyA2);
    
    %basal synapses
    % \node[below left=1.0cm and .5cm of z1] (z1B1) {};
    % \path[-, thick] ([xshift=-.25cm] z1.south west) edge (z1B1);
    \node[below left=1.0cm and .2cm of z1] (z1B2) {};
    \path[-, thick] ([xshift=-.25cm] z1.south west) edge (z1B2);
    \node[bsynapse] at (intersection of [xshift=-.25cm] z1.south west--z1B2 and b3--b3R) {};
    \node[bsynapse] at (intersection of [xshift=-.25cm] z1.south west--z1B2 and b2--b2R) {};
    \node[bsynapse] at (intersection of [xshift=-.25cm] z1.south west--z1B2 and b1--b1R) (bs1) {};
    % \node[above left=.01cm and -.15cm of bs1] {${\color{blue}b_1}$};

    \node[below left=1.0cm and .2cm of zd] (zdB1) {};
    \path[-, thick] ([xshift=-.25cm] zd.south west) edge (zdB1);
    % \node[below left=1.0cm and .5cm of zd] (zdB2) {};
    % \path[-, thick] ([xshift=-.25cm] zd.south west) edge (zdB2);
    \node[bsynapse] at (intersection of [xshift=-.25cm] zd.south west--zdB1 and b3--b3R) {};
    \node[bsynapse] at (intersection of [xshift=-.25cm] zd.south west--zdB1 and b2--b2R) {};
    \node[bsynapse] at (intersection of [xshift=-.25cm] zd.south west--zdB1 and b1--b1R) (bsk) {};
    % \node[above left=.01cm and -.15cm of bsk] {${\color{blue}b_k}$};

    %\node[below right=0.9cm and .2cm of z1] (z1I1) {};
    %\path[-, thick] ([xshift=.25cm] z1.south east) edge (z1I1);
    % \node[below right=1.8cm and -.15cm of z1] (z1I2) {};
    % \path[-, thick] ([xshift=.25cm] z1.south east) edge (z1I2);
    % \node[isynapse] at (intersection of [xshift=.25cm] z1.south east--z1I2 and i3--i3R) {};
    \node[isynapse] at (intersection of  z1--z1A and i2--i2R) {};
    \node[isynapse] at (intersection of  z1--z1A and i1--i1R) {};
    
    
    %\node[bsynapse] at (intersection of [xshift=.25cm] z1.south east--z1I1 and b2--b2R) {};

    % \node[below right=1.0cm and .45cm of zd] (zdI1) {};
    % \path[-, thick] ([xshift=.25cm] zd.south east) edge (zdI1);
    %\node[below right=1.0cm and .2cm of zd] (zdI2) {};
    %\path[-, thick] ([xshift=.25cm] zd.south east) edge (zdI2);
    % \node[isynapse] at (intersection of [xshift=.25cm] zd.south east--zdI2 and i3--i3R) {};
    \node[isynapse] at (intersection of zd--zdA and i2--i2R) {};
    \node[isynapse] at (intersection of zd--zdA and i1--i1R) {};
    %\node[bsynapse] at (intersection of [xshift=.25cm] zd.south east--zdI2 and b2--b2R) {};
    
    %axon to interneuron
    \node[below left=0.8cm and -.25cm of int1] (int1S) {};
    \node[below right=0.8cm and -.25cm of int2] (int2S) {};
    % \node[below right=0.9cm and -.15cm of int3] (int3S) {};
    
    \path[-,  black!30!green, thick] (int1.south) edge (int1S);
    \path[-,  black!30!green, thick] (int2.south) edge (int2S);
    % \path[-,  black!30!green, thick] (int3.south) edge (int3S);

    \node[psynapse] at (intersection of int1.south--int1S and z1Axon--pyA1) {};
    \node[psynapse] at (intersection of int1.south--int1S and zdAxon--pyA2) {};
    \node[psynapse] at (intersection of int2.south--int2S and z1Axon--pyA1) {};
    \node[psynapse] at (intersection of int2.south--int2S and zdAxon--pyA2) {};
    % \node[psynapse] at (intersection of int3.south--int3S and z1Axon--pyA1) {};
    % \node[psynapse] at (intersection of int3.south--int3S and zdAxon--pyA2) {};
    
    \node[asynapse] at (2.15,-4.0) (p) {}; 
    \node[right=0.07cm of p] (atext) {\scriptsize $\!\V_{\!y}^\top$};
    \node[psynapse] at (2.15,-4.4) (a) {};
    \node[right=0.07cm of a] (ptext) {\scriptsize $\Q$};
    \node[bsynapse] at (3.3,-4.0) (b) {};
    \node[right=0.07cm of b] (btext) {\scriptsize $\!\V_{\!x}^\top\!$};
    \node[isynapse] at (3.3,-4.4) (i) {};
    \node[right=0.07cm of i] (itext) {\scriptsize $\!\!\Q^\top\!$};
    \draw[rounded corners=0.2,color=black!50] (1.9,-3.785) rectangle (4.1,-4.605);
\end{tikzpicture}

==> old-stuff/old-sections/algo_der.tex <==

In this section, starting from Eq.~\eqref{eq:genrrr2}, we derive offline and online algorithms for the family of RRR objectives parametrized by $s$.

\subsection{Offline algorithms}

Noting that imposing the constraint $\V_x^\top\C_{xx}\V_x=\I_k$ via a Lagrange multiplier
% (as in Sec.~\ref{app:CCA_from_grrr}) 
leads to non-local update rules (see Sec.~\ref{app:naive_bio} of the supplementary materials), following \cite{pehlevan2015normative} we  impose the weaker inequality constraint $\V_x^\top\C_{xx}\V_x  \preceq \I_k$ by introducing the matrix $\Q\in\R^{k \times k}$
\begin{equation}\label{eq:genrrr_final}
    \min_{\V_x\in\R^{m\times k}}\min_{\V_y\in\R^{n\times k}}\max_{\Q\in\R^{k \times k}} \tr\V_y^\top\Sig^{-1}_s\V_y-2\V_x^\top\C_{xy}\V_y+\Q\Q^\top(\V_x^\top\C_{xx}\V_x-\I_k),
\end{equation}
where $\Q\Q^\top$ is the positive semi-definite Lagrange multiplier enforcing the inequality. As in~\cite{pehlevan2015normative}, the dynamics of the optimization enforce that the inequality constraint is saturated, i.e. $\V_x^\top\C_{xx}\V_x=\I_k$ is satisfied at the optimum of the objective (for a different proof see Sec.~\ref{app:rrr_sol_details}). This objective can be optimized using gradient descent-ascent dynamics derived by taking partial derivatives:
\begin{align}
    \V_x^\top&\gets\V_x^\top+\eta(\V_y^\top \C_{yx}-\Q\Q^\top\V_x^\top\C_{xx})\label{eq:Vx_offline}\\
    \V_y^\top&\gets\V_y^\top+\eta(\V_x^\top \C_{xy}-\V_y^\top\Sig^{-1}_s)\label{eq:Vy_offline}\\
    \Q&\gets\Q+\frac{\eta}{\tau}(\V_x^\top\C_{xx}\V_x-\I_k)\Q,\label{eq:Q_offline}
\end{align}
where $\eta>0$ is the learning rate for $\V_x$ and $\V_y$, and $\tau>0$ is a parameter controlling the ratio of the descent and ascent steps.


\subsection{Online algorithms} \label{sec:rrr}

In the online (or streaming) setting, input is  presented one sample at a time and the algorithm must find the projection without storing any significant fraction of the dataset. %process the desired projection and update the weights of the algorithm while having access to this one sample alone. 

% \paragraph{RRR ($\Sig=\I_k$).}~ 
To derive an online algorithm, we rewrite the objective function~\eqref{eq:genrrr_final} making the dependence of the objective on each individual sample manifest:
% \begin{multline}
%     \min_{\V_x\in\R^{m\times k}}\min_{\V_y\in\R^{n\times k}}\max_{\Q\in\R^{k\times k}}\frac1T\sum_{t=1}^T \V_y^\top(s \y \y^\top + (1-s)\I_n)\V_y-2\V_x^\top\x_t\y_t^\top\V_y\\+\Q\Q^\top(\V_x^\top\x_t\x_t^\top\V_x-\I_k),
% \end{multline}
\begin{equation}
    \min_{\V_x}\min_{\V_y}\max_{\Q}\frac1T\sum_{t=1}^T \V_y^\top(s \y \y^\top + (1-s)\I_n)\V_y-2\V_x^\top\x_t\y_t^\top\V_y+\Q\Q^\top(\V_x^\top\x_t\x_t^\top\V_x-\I_k).
\end{equation}
% where we have defined 
% \begin{equation}
%     \S_t := \left\{\begin{array}{lr}
%         \I_n & \text{(RRMSE)} \\
%         \y_t \y_t^\top  & \text{(CCA)} \end{array}\right.
% \end{equation}
% such that $\Sig=\frac1T\sum_{t=1}^T\S_t$.
If we now perform stochastic gradient descent/ascent~\cite{SGD}, i.e.~perform the gradient updates with respect to individual samples, we arrive at our online algorithm. Explicitly, at time $t$ we have:
\begin{align}
    \V_x^\top&\gets\V_x^\top+\eta(\a_t-\Q\n_t)\x_t^\top\label{eq:Vx_circuit}\\
    % \V_y^\top&\gets\V_y^\top+\eta\left\{\begin{array}{lr}
    %     \hspace{-5pt}(\z_t\y_t^\top-\V_y^\top) & \text{(RRMSE)} \label{eq:Vy_circuit}\vspace{2.5pt}\\
    %     \hspace{-5pt}(\z_t-\a_t)\y_t^\top & \text{(CCA)} \end{array}\right.\\
    \V_y^\top&\gets\V_y^\top+\eta (\z_t\y_t^\top -s\, \a_t\y_t^\top - (1-s)\,\V_y^\top)\label{eq:Vy_circuit}\\
    \Q&\gets\Q+\frac{\eta}{\tau}(\z_t\n_t^\top-\Q)\label{eq:Q_circuit}.
\end{align}
% \begin{align}
%     \V_x^\top&\gets\V_x^\top+\eta(\a_t-\Q\n_t)\x_t^\top\\
%     \V_y^\top&\gets\V_y^\top+\eta(\z_t\y_t^\top-\V_y^\top)\\
%     \Q&\gets\Q+\frac{\eta}{\tau}(\z_t\n_t^\top-\Q),
% \end{align}
where  $\z_t:=\V_x^\top\x_t$ is the output of the algorithm, $\a_t:=\V_y^\top\y_t$ and $\n_t:=\Q^\top\z_t$.
% 
% \paragraph{CCA ($\Sig=\C_{yy})$.} The derivation in this case proceeds similarly. We rewrite the objective function~\eqref{eq:genrrr_final} to make the dependence on each sample explicit:
% \begin{multline}
%     \min_{\V_x\in\R^{m\times k}}\min_{\V_y\in\R^{n\times k}}\max_{\Q\in\R^{k\times k}}\frac1T\sum_{t=1}^T\V_y^\top\y_t\y_t^\top\V_y-2\V_x^\top\x_t\y_t^\top\V_y\\+\Q\Q^\top(\V_x^\top\x_t\x_t^\top\V_x-\I_k).
% \end{multline}
% At time $t$, the iterative SGD update is given by:
% \begin{align}
%     \V_x^\top&\gets\V_x^\top+\eta(\a_t-\Q\n_t)\x_t^\top\\
%     \V_y^\top&\gets\V_y^\top+\eta(\z_t-\a_t)\y_t^\top\\
%     \Q&\gets\Q+\frac{\eta}{\tau}(\z_t\n_t^\top-\Q),
% \end{align}
% with $\z_t$, $\a_t$ and $\n_t$ as above. 
% 
% Here we just note that the algorithm is local: the update rule for any synapse $S_{ij}$ connecting neurons $i$ and $j$ only depends on itself and the synaptic weight modulated neural activity of the adjacent neurons (e.g. $\a_t=\V_y^\top \y_t$ or $\Q\n_t$). These are all all locally available to the neuron.

% 
Our RRR algorithms, which we call Bio-RRR, in the offline and online setting are summarized in Alg.~\ref{alg:cca_offline} and Alg.~\ref{alg:cca_online}. 
% For online algorithms, the computational complexity per iteration is $\mathcal O((m+n)k+k^2)$. This compares favorably with competing (non-biological) algorithms for RRMSE~\cite{RRR_MLE,IQMD,hua2001optimal,RRR_robust,ORRR} and (multi-component) CCA~\cite{arora2017stochastic, lai1999neural, pezeshki2003network, via2007learning, haga2017dendritic} with scaling of at least \mbox{$\mathcal O((m+n)^2)$}.

\input{algos}

==> old-stuff/old-sections/algos.tex <==
% \setlength{\columnsep}{18pt}%
% \setlength{\intextsep}{1pt}
\begin{figure}[ht]
% \begin{wrapfigure}{r}{0.425\textwidth}
% \vspace{-10pt}
\centering
\begin{minipage}{0.481\textwidth}
\begin{algorithm}[H]
  \caption{\hspace{-2.5pt}\textbf{: } Offline Bio-RRR 
%   \\\textbf{Algorithm 2b: } Offline Bio-CCA 
  }
  \label{alg:cca_offline}
\begin{algorithmic}
  \STATE \hspace{-6pt}{\bfseries input:} $\X\in\R^{m\times T}$, $\Y\in\R^{n\times T}$% dimension $k$
  \STATE \hspace{-6pt}{\bfseries initialize} $\V_x$, $\V_y$, and $\Q$.
  \STATE \hspace{-6pt}$\C_{xx}\gets \X\X^\top/T \; ; \; \C_{xy}\gets \X\Y^\top/T$\vspace{1pt}
%   \STATE \hspace{-6pt}$\Sig\gets\left\{\begin{array}{lc}
%         \I_n & \text{(RRMSE)} \\
%         \Y\Y^\top/T \;\;\;\;& \text{(CCA)} \end{array}\right.$
  \STATE \hspace{-6pt}$\Sig_s^{-1}\gets s\,\Y\Y^\top/T +(1-s)\,\I_n$
  \STATE \hspace{-6pt}{\bfseries repeat:}\vspace{2pt}
  \STATE \hspace{3pt}\mbox{$\V_x^\top\gets\V_x^\top+\eta(\V_y^\top \C_{yx}-\Q\Q^\top\V_x^\top\C_{xx})$} \vspace{1pt}
  \STATE \hspace{3pt}$\V_y^\top\gets\V_y^\top+\eta(\V_x^\top \C_{xy}-\V_y^\top\Sig_s^{-1})$ \vspace{2pt}
  \STATE \hspace{3pt}$\Q\gets\Q+\frac{\eta}{\tau}(\V_x^\top\C_{xx}\V_x-\I_k)\Q$ \vspace{2pt}
  \STATE \hspace{-6pt}{\bfseries until} convergence
  \STATE \hspace{-6pt}{\bfseries output:}  $\Z=\V_x^\top \X$ \hfill $\triangleright\;$ projected predictor
\end{algorithmic}
\end{algorithm}
\end{minipage}
% 
\hfill
% 
\begin{minipage}{0.481\textwidth}
\begin{algorithm}[H]\vspace{2pt}
  \caption{\hspace{-2.5pt}\textbf{: } Online Bio-RRR
%   \\\textbf{Algorithm 2b: } Online Bio-CCA 
}
  \label{alg:cca_online}
\begin{algorithmic}%\vspace{-1pt}
  \STATE \hspace{-4pt}{\bfseries input:} $\x_t\in\R^m$, $\y_t\in\R^n$ \hfill $\triangleright\;$ new sample \vspace{2pt}
  \\\hspace{24pt} $\V_x, \V_y, \Q$ \hfill $\triangleright\;$ previous matrices\vspace{3pt}
%   \STATE \hspace{-6pt}{\bfseries initialize} $\V_x$, $\V_y$, and $\Q$.
%   \STATE \hspace{-6pt}{\bfseries for} $t=1, 2,\dots,T $ {\bfseries do:}
%   \STATE \hspace{2pt}Draw sample $(\x_t,\y_t)$ from $(\X,\Y)$
  \STATE \hspace{-4pt}$\z_t\gets\V_x^\top\x_t;\quad\n_t\gets\Q^\top\z_t;\quad \a_t\gets\V_y^\top\y_t$ \vspace{5pt}
%   \STATE \hspace{2pt}Gradient descent-ascent step:
  \STATE \hspace{-4pt}$\V_x^\top\gets\V_x^\top+\eta(\a_t-\Q\n_t)\x_t^\top$ \vspace{5pt}
%   \STATE \mbox{\hspace{-4pt}$\V_y^\top\gets\V_y^\top+\eta\left\{\begin{array}{lc}
%         \hspace{-5pt}(\z_t\y_t^\top-\V_y^\top) & \text{(RRMSE)} \vspace{2pt}\\
%         \hspace{-5pt}(\z_t-\a_t)\y_t^\top & \text{(CCA)} \end{array}\right.$} \vspace{3pt}
  \STATE \hspace{-4pt}$\V_y^\top\gets\V_y^\top+\eta(\z_t\y^\top -s\, \a_t\y^\top - (1-s)\,\V_y^\top)$ \vspace{-2pt}
  \STATE \hspace{-4pt}$\Q \gets\Q+\frac{\eta}{\tau}(\z_t\n_t^\top-\Q) $ \vspace{4pt}
%   \STATE \hspace{-6pt}{\bfseries end for}
  \STATE \hspace{-4pt}{\bfseries output:}  $\z_t$ \hfill $\triangleright\;$ projected sample\vspace{3pt}
  \\\hspace{27pt} $\V_x, \V_y, \Q$ \hfill $\triangleright\;$ updated matrices
\end{algorithmic}
\end{algorithm}
\end{minipage}
% \vspace{-15pt}
% \end{wrapfigure}
\end{figure}

% {\bf DL: I wonder if this is too compact. Here is a alternate display of the algorithms:}

% Offline algorithms:

% % \setlength{\columnsep}{18pt}%
% % \setlength{\intextsep}{1pt}
% \begin{figure}[ht]
% % \begin{wrapfigure}{r}{0.425\textwidth}
% % \vspace{-10pt}
% \centering
% \begin{minipage}{0.481\textwidth}
% \begin{algorithm}[H]
%   \caption{Offline RRR}
%   \label{alg:cca_offline}
% \begin{algorithmic}
%   \STATE \hspace{-6pt}{\bfseries input:} data  $\X\in\R^{m\times T}$, $\Y\in\R^{n\times T}$% dimension $k$
%   \STATE \hspace{-6pt}{\bfseries initialize} $\V_x$, $\V_y$, and $\Q$.
%   \STATE \hspace{-6pt}$\C_{xx}\gets \X\X^\top/T$
%   \STATE \hspace{-6pt}$\C_{xy}\gets \X\Y^\top/T$
%   \STATE \hspace{-6pt}{\bfseries repeat:}\vspace{2pt}
%   \STATE \hspace{3pt}\mbox{$\V_x^\top\gets\V_x^\top+\eta(\V_y^\top \C_{yx}-\Q\Q^\top\V_x^\top\C_{xx})$} \vspace{1pt}
%   \STATE \hspace{3pt}$\V_y^\top\gets\V_y^\top+\eta(\V_x^\top \C_{xy}-\V_y^\top)$ \vspace{2pt}
%   \STATE \hspace{3pt}$\Q\gets\Q+\frac{\eta}{\tau}(\V_x^\top\C_{xx}\V_x-\I_k)\Q$ \vspace{2pt}
%   \STATE \hspace{-6pt}{\bfseries until} convergence
%   \STATE \hspace{-6pt}{\bfseries output:} matrices $\V_x$, $\V_y$
% \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% % 
% \hfill
% % 
% \begin{minipage}{0.481\textwidth}
% \begin{algorithm}[H]\vspace{2pt}
%   \caption{Offline CCA}
%   \label{alg:cca_offline}
% \begin{algorithmic}
%   \STATE \hspace{-6pt}{\bfseries input:} data  $\X\in\R^{m\times T}$, $\Y\in\R^{n\times T}$% dimension $k$
%   \STATE \hspace{-6pt}{\bfseries initialize} $\V_x$, $\V_y$, and $\Q$.
%   \STATE \hspace{-6pt}$\C_{xx}\gets \X\X^\top/T \; , \; \C_{yy}\gets \Y\Y^\top/T$
%   \STATE \hspace{-6pt}$\C_{xy}\gets\X\Y^\top/T.$
%   \STATE \hspace{-6pt}{\bfseries repeat:}\vspace{2pt}
%   \STATE \hspace{3pt}\mbox{$\V_x^\top\gets\V_x^\top+\eta(\V_y^\top \C_{yx}-\Q\Q^\top\V_x^\top\C_{xx})$} \vspace{1pt}
%   \STATE \hspace{3pt}$\V_y^\top\gets\V_y^\top+\eta(\V_x^\top \C_{xy}-\V_y^\top\C_{yy})$ \vspace{2pt}
%   \STATE \hspace{3pt}$\Q\gets\Q+\frac{\eta}{\tau}(\V_x^\top\C_{xx}\V_x-\I_k)\Q$ \vspace{2pt}
%   \STATE \hspace{-6pt}{\bfseries until} convergence
%   \STATE \hspace{-6pt}{\bfseries output:} matrices $\V_x$, $\V_y$
% \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% % \vspace{-15pt}
% % \end{wrapfigure}
% \end{figure}

% Online algorithms:

% % \setlength{\columnsep}{18pt}%
% % \setlength{\intextsep}{1pt}
% \begin{figure}[ht]
% % \begin{wrapfigure}{r}{0.425\textwidth}
% % \vspace{-10pt}
% \centering
% \begin{minipage}{0.481\textwidth}
% \begin{algorithm}[H]
%   \caption{Online RRR\vspace{1pt}}
%   \label{alg:cca_online}
% \begin{algorithmic}\vspace{-1pt}
%   \STATE \hspace{-6pt}{\bfseries input:} data  $\X\in\R^{m\times T}$, $\Y\in\R^{n\times T}$% dimension $k$
%   \STATE \hspace{-6pt}{\bfseries initialize} $\V_x$, $\V_y$, and $\Q$.
%   \STATE \hspace{-6pt}{\bfseries for} $t=1, 2,\dots,T $ {\bfseries do:}
%   \STATE \hspace{2pt}Draw sample $(\x_t,\y_t)$ from $(\X,\Y)$
%   \STATE \hspace{2pt}$\z_t\gets\V_x^\top\x_t,\quad\n_t\gets\Q^\top\z_t$ \vspace{2pt}
% %   \STATE \hspace{2pt}Gradient descent-ascent step:
%   \STATE \hspace{2pt}$\V_x^\top\gets\V_x^\top+\eta(\V_y^\top \y_t-\Q\n_t)\x_t^\top$
%   \STATE \hspace{2pt}$\V_y^\top\gets\V_y^\top+\eta(\z_t\y_t^\top-\V_y^\top)$
%   \STATE \hspace{2pt}$\Q \gets\Q+\frac{\eta}{\tau}(\z_t\n_t^\top-\Q). $ \vspace{2pt}
%   \STATE \hspace{-6pt}{\bfseries end for}
%   \STATE \hspace{-6pt}{\bfseries output:}  matrices $\V_x$, $\V_y$
% \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% % 
% \hfill
% % 
% \begin{minipage}{0.481\textwidth}
% \begin{algorithm}[H]\vspace{2pt}
%   \caption{Online CCA\vspace{1pt}}
%   \label{alg:cca_online}
% \begin{algorithmic}\vspace{-1pt}
%   \STATE \hspace{-6pt}{\bfseries input:} data  $\X\in\R^{m\times T}$, $\Y\in\R^{n\times T}$% dimension $k$
%   \STATE \hspace{-6pt}{\bfseries initialize} $\V_x$, $\V_y$, and $\Q$.
%   \STATE \hspace{-6pt}{\bfseries for} $t=1, 2,\dots,T $ {\bfseries do:}
%   \STATE \hspace{2pt}Draw sample $(\x_t,\y_t)$ from $(\X,\Y)$
%   \STATE \hspace{2pt}$\z_t\gets\V_x^\top\x_t,\quad\n_t\gets\Q^\top\z_t$ \vspace{2pt}
% %   \STATE \hspace{2pt}Gradient descent-ascent step:
%   \STATE \hspace{2pt}$\V_x^\top\gets\V_x^\top+\eta(\V_y^\top \y_t-\Q\n_t)\x_t^\top$
%   \STATE \hspace{2pt}$\V_y^\top\gets\V_y^\top+\eta(\z_t-\V_y^\top\y_t)\y^\top$
%   \STATE \hspace{2pt}$\Q \gets\Q+\frac{\eta}{\tau}(\z_t\n_t^\top-\Q). $ \vspace{2pt}
%   \STATE \hspace{-6pt}{\bfseries end for}
%   \STATE \hspace{-6pt}{\bfseries output:}  matrices $\V_x$, $\V_y$
% \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% % \vspace{-15pt}
% % \end{wrapfigure}
% \end{figure}

==> old-stuff/old-sections/backprop.tex <==





Experimentally, calcium plateau potentials act as instructive signals in cortical pyramidal neurons by driving plasticity in the proximal dendrites~\cite{bittner2017behavioral,GreinbergerMagee2020,Milstein2020}.
In an attempt to find a biologically plausible implementation of the backpropagation algorithm, a recent work~\cite{Payeur2020} suggested that the calcium plateau potential carries the backpropagation error. Here, we show the that calcium plateau potential  plays a similar role in Bio-RRR provided the network is close to the optimum of the objective. To this end, we compare the Bio-RRR $\V_x^\top$ learning rule, which relies on the calcium plateau potential, with that of the first layer weights of a two-layer artificial neural network (ANN) which optimizes Eq.~\eqref{eq:genrrr1}.



% It has been suggested that the calcium plateau potential is involved in error backpropagation in biological neural networks~\cite{Payeur2020}. 
% Here, we demonstrate how this is explicitly realized in the Bio-RRR algorithm.
% 
% Recently, ~\cite{Payeur2020} showed using numerical simulations that when synaptic plasticity is regulated by high-frequency bursts of spikes, downstream cortical regions can backpropagate error signal as would be necessary in deep networks. The results in our paper are a natural complement to~\cite{Payeur2020}, as we derive the synaptic plasticity rules of the micro-circuits in a normative way. These micro-circuits could then be stacked into a deep network as proposed in ~\cite{Payeur2020}.
% 
% To this end, it is instructive to consider a two-layer artificial neural network (ANN) implementation of the RRR objective (given in Eq.~\ref{eq:genrrr1}), and compare the ANN learning rule for $\V_x^\top$ to that of Bio-RRR, which we showed in the previous section is driven by the calcium plateau potential.


A cartoon of an ANN optimizing the RRR objective in Eq.~\eqref{eq:genrrr1}, is given in Fig.~\ref{fig:rrr_ann} where we have set $\Sig=\I_n$ for simplicity. 
Here, the forward and backward passes of the network are respectively denoted by blue and red arrows, and $\hat \y_t = \V_y\V_x^\top \x_t$ is the network's inferred value of the response~$\y_t$.
% based on the predictor variable $\x_t$. 
% 
The updates for $\V_x^\top$ and $\V_y$, the weights of the first and second layer of the ANN, require the computation and backpropagation of the error signal $\boldsymbol{\epsilon}_t = \y_t - \hat \y_t$. In particular, the update for $\V_x^\top$ is proportional to the covariance of the backpropagated error signal $\V_y^\top \boldsymbol{\epsilon}_t$ and the input $\x_t^\top$. 


A cartoon of the implementation of the Bio-RRR algorithm is given in Fig.~\ref{fig:rrr_bio}. Here, the inferred value $\hat \y_t$ and the error signal $\boldsymbol{\epsilon}_t = \y_t - \hat \y_t$ are not computed. However, the update for $\V_x^\top$ can still be interpreted intuitively in the context of error backpropagation. To make this connection manifest, we look at the optimum of the objective where, from Eq.~\eqref{eq:Vx_offline}, we have
\begin{equation*}
    \Q\Q^\top\V_x^\top = \V_y^\top\C_{yx}\C_{xx}^{-1}\;%, \quad \Z \Z^\top = \I_n.
    \;\Rightarrow\;
    \Q\n_t = \Q\Q^\top\V_x^\top \x_t =  \V_y^\top\C_{yx}\C_{xx}^{-1} \x_t = \V_y^\top \tilde\y_t,
\end{equation*}
where we have used $\n_t=\Q^\top\z_t$ and $\z_t=\V_x^\top\x_t$, and we have defined $\tilde\y_t := \C_{yx}\C_{xx}^{-1} \x_t$.
As \mbox{$\C_{yx} \C_{xx}^{-1}=\text{arg$\,$min}_\W \lVert\Y-\W\X\rVert^2_{\Sig}$} is the optimum of the rank-unconstrained regression objective, $\tilde\y_t$ is the best estimate of $\y_t$ given the samples received thus far. Using these quantities and the definition of $\a_t = \V_y^\top \y_t$, we can rewrite the quantity $\a_t-\Q\n_t$ and the $\V_x^\top$ update in Eq.~\eqref{eq:Vx_circuit} as
\begin{align}
    \a_t - \Q\n_t = \V_y^\top (\y_t-\tilde\y_t)\quad\Rightarrow\quad
    \V_x^\top&\gets\V_x^\top+\eta\;\Big[\V_y^\top(\!\underbrace{\,\y_t-\tilde\y_t}_{\text{prediction error}}\!)\,\Big]\x_t^\top \label{eq:Vx_at_equil}.
\end{align}
Therefore, while the error term $\y_t-\tilde\y_t$ and backpropagation are not present explicitly in Bio-RRR, at the optimum, the calcium plateau potential is equal to a backpropagated error signal, and the update of $\V_x^\top$ is proportional to the covariance of this backpropagated error signal and the input $\x_t^\top$. 

Finally, Bio-RRR offers a solution to a difficulty encountered in biological implementations of backpropagation in that the computation of the $\V_x$ update in the ANN requires the use of $\V_y$ in the forward pass and its transpose $\V_y^\top$ in the backward pass. This symmetry between the forward and backward weights is a general property of SGD in deep networks but is not biologically realistic and is referred to as the weight transport problem~\cite{weight_transport_problem1,weight_transport_problem2,weight_transport_problem3}. Several solutions exist to facilitate the backpropagation of the computed error in a biologically plausible manner~\cite{Burbank2012,Burbank2015,Lillicrap2016,Akrout2019}. In Bio-RRR, the inferred value $\hat \y_t$ and the error signal $\boldsymbol{\epsilon}_t = \y_t - \hat \y_t$ are not computed explicitly, and the weights $\V_y^\top$ are only used once. Since there is no explicit error computation and backpropagation, we circumvent the weight transport problem altogether.\footnote{As mentioned in Sec.~\ref{sec:circuit}, the weights $\Q$ and $\Q^\top$ can be decoupled without affecting the Bio-RRR algorithm. See Sec.~\ref{app:decoupled_weights} of the supplementary materials for details.}

==> old-stuff/old-sections/cca.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  CCA algorithm %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The derivation in this case proceeds similarly. We rewrite the objective function \eqref{eq:genrrr_final} to make the dependence on each sample explicit:
\begin{multline}
    \min_{\V_x\in\R^{m\times k}}\min_{\V_y\in\R^{n\times k}}\max_{\Q\in\R^{k\times k}}\frac1T\sum_{t=1}^T\V_y^\top\y_t\y_t^\top\V_y-2\V_x^\top\x_t\y_t^\top\V_y\\+\Q\Q^\top(\V_x^\top\x_t\x_t^\top\V_x-\I_k).
\end{multline}
At time $t$, the iterative SGD update is given by:
\begin{align}
    \V_x^\top&\gets\V_x^\top+\eta(\a_t-\Q\n_t)\x_t^\top\\
    \V_y^\top&\gets\V_y^\top+\eta(\z_t-\a_t)\y_t^\top\\
    \Q&\gets\Q+\frac{\eta}{\tau}(\z_t\n_t^\top-\Q),
\end{align}
where
\begin{align}
    \a_t:=\V_y^\top\y_t,&&\z_t:=\V_x^\top\x_t,&&\n_t:=\Q^\top\z_t=\Q^\top\V_x^\top\x_t.
\end{align}

% The derivation of the CCA algorithm follows in the same vein as RRR. Starting from the objective function~\eqref{eq:CCA_first}
% % \begin{equation*}
% %     \min_{\V_x\in\R^{m\times d}}\min_{\V_y\in\R^{n\times d}}\tr\V_y^\top\Y\Y^\top\V_y-2\V_x^\top\X\Y^\top\V_y,\quad\text{subject to}\;\V_x^\top\X\X^\top\V_x=\I_d,
% % \end{equation*}
% we again impose the inequality $\V_x^\top\X\X^\top\V_x  \preceq \I_k$ via the matrix $\Q\in\R^{k\times K}$
% \begin{equation}\label{eq:cca_final}
%     \min_{\V_x\in\R^{m\times k}}\min_{\V_y\in\R^{n\times k}}\max_{\Q\in\R^{k \times k}} \tr\V_y^\top\C_{yy}\V_y-2\V_x^\top\C_{xy}\V_y+\Q\Q^\top(\V_x^\top\C_{xx}\V_x-\I_k),
% \end{equation}
% where again the inequality is saturated due to the dynamics of the optimization~\cite{pehlevan2015normative}. We optimize this objective using gradient descent-ascent equations:
% \begin{align}\label{eq:cca_offline_updates}
%     \V_x^\top&\gets\V_x^\top+\eta(\V_y^\top \C_{yx}-\Q\Q^\top\V_x^\top\C_{xx})\notag\\
%     \V_y^\top&\gets\V_y^\top+\eta(\V_x^\top \C_{xy}-\V_y^\top\C_{yy})\\
%     \Q&\gets\Q+\frac{\eta}{\tau}(\V_x^\top\C_{xx}\V_x-\I_k)\Q.\notag
% \end{align}

% \paragraph{Online algorithm.} 
% Using the variables $\Z$ and $\N$ defined as in the RRR algorithm, we can derive the online CCA algorithm using stochastic gradients. The update rules at time $t$ are
% \begin{align}\label{eq:cca_online_updates}
%     \V_x^\top&\gets\V_x^\top+\eta(\V_y^\top \y_t-\Q\n_t)\x_t^\top\notag\\
%     \V_y^\top&\gets\V_y^\top+\eta(\z_t-\V_y^\top \y_t)\y_t^\top\\
%     \Q&\gets\Q+\frac{\eta}{\tau}(\z_t\n_t^\top-\Q).\notag
% \end{align}
Similar to the RRR updates in Eq.~\eqref{eq:rrr_online_updates}, these update rules are comprised only of variables locally available to the neuron. The RRR and CCA algorithms in the offline and online setting are summarized in Alg.~\ref{alg:cca_offline} and Alg.~\ref{alg:cca_online}. In each case, the difference between the RRR and CCA algorithm is only in one line of the algorithm, which is accordingly demarcated. 

We finally note that the computational complexity of our algorithm per iteration in both RRR and CCA in the online scenario is $\mathcal O((m+n)k+k^2)$. This compares favorably with competing (non-biological) algorithms for RRR and (multi-component) CCA with scalings $\geq \mathcal O(m^2)$.

\input{algos}




==> old-stuff/old-sections/experiments.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  numerics %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section we report the results of numerical simulations for our algorithms with $s=0$ denoted as Bio-RRMSE and $s=1$ denoted as Bio-CCA, and compare with current non-biologically plausible algorithms.
For our experiments we use the MediaMill dataset~\cite{snoek2006challenge}, a commonly used  real-world benchmark consisting of $T=2\times10^4$ samples of video data and text annotations. For our experiments, we take the predictor variables $\X$ to be the 100-dimensional textual features and the response variable to be the 120-dimensional visual features extracted from representative video frames.

\begin{figure}[ht]
\vspace{-10pt}
\centering
\includegraphics[width=\textwidth]{main_results.pdf}
\caption{\small Comparisons of RRR algorithms for (a) RRMSE ($s=0$) and (b) CCA ($s=1$) in terms of the objective value Eq.~\eqref{eq:genrrr2} vs. iteration and runtime.  Mean $\pm$ standard deviation over 5 runs of the experiment.}
\label{fig:RRR_comparison} 
\vspace{-5pt}
\end{figure}

\paragraph{RRMSE.} The performance of our RRMSE algorithm on MediaMill is given in Fig.~\ref{fig:RRR_comparison}{\color{blue}a} in terms of the objective function in Eq.~\eqref{eq:genrrr2} with $\Sig = \I_n$. For ranks  $k \in \{1, 2, 4\}$, we plot this both as a function of iteration (top) and as a function of the CPU runtime (bottom). Here, the black dashed line denotes the value of the objective at its global minimum.  For comparison, we provide the performance of the iterative quadratic minimum distance (IQMD) algorithm~\cite{IQMD} and the 2-layer ANN discussed in Sec.~\ref{sec:backprop}. We see that IQMD is the most sample efficient, and ANN and Bio-RRMSE are within variance of each other and match the performance of IQMD in runtime. For plots of these algorithms in the offline (batch) setting see Sec.~\ref{app:exp_details}.

\paragraph{CCA.} We evaluate the performance of our CCA algorithm on the MediaMill dataset and compare with CCALin~\cite{ge2016efficient} and SAA~\cite{Gao2019CCA} which are offline algorithms, and MSG-CCA~\cite{arora2017stochastic} which is online. In Fig.~\ref{fig:RRR_comparison}{\color{blue}b}, we plot the performance of the different algorithms for CCA projection dimensions $k\in\{1,2,4\}$ in terms of the objective function given in Eq.~\eqref{eq:genrrr2}. We see that on this dataset, our offline algorithm (Bio-CCA - offline) is the most sample efficient and our online algorithm (Bio-CCA - online) is fastest in terms of CPU runtime. 
% Again, the different scaling of the various algorithms would make Bio-CCA even more competitive  as input dimension is increased. 

% \begin{figure}[ht]
% \vspace{-5pt}
% \centering
% \subfloat[$k=1$]{\label{figur:rank_1_iter_MMill2}
% \begin{minipage}{.32\textwidth}
% \centering
% \includegraphics[trim={4 2 27 17},clip,width=\textwidth]{figures/k1itmmm_newob.pdf}\\\includegraphics[trim={4 2 27 2},clip,width=\textwidth]{k1rtmmm_newob.pdf}
% \end{minipage}} 
% \hspace{1.5pt}
% \subfloat[$k=2$]{\label{figur:rank_2_iter_MMill2}
% \begin{minipage}{.32\textwidth}
% \centering\includegraphics[trim={4 2 27 17},clip,width=\textwidth]{k2itmmm_newob.pdf}\\\includegraphics[trim={4 2 27 2},clip,width=\textwidth]{k2rtmmm_newob.pdf}
% \end{minipage}} 
% \hspace{1.5pt}
% \subfloat[$k=4$]{\label{figur:rank_4_iter_MMill2}
% \begin{minipage}{.32\textwidth}
% \centering\includegraphics[trim={4 2 27 17},clip,width=\textwidth]{k4itmmm_newob.pdf}\\\includegraphics[trim={4 2 27 2},clip,width=\textwidth]{k4rtmmm_newob.pdf}
% \end{minipage}} 
% \includegraphics[width=\textwidth]{CCA_combined_results.pdf}
% \caption{\small Comparisons of our CCA algorithm in the online and offline setting with CAPPED-MSG~\cite{arora2017stochastic}, CCALin~\cite{ge2016efficient} and SAA~\cite{Gao2019CCA} algorithms on the MediaMill data set~\cite{snoek2006challenge}, in terms of the objective value Eq.~\eqref{eq:genrrr2} as a function of iteration (top) and as a function of CPU runtime (bottom) averaged over 4 runs of the experiment.} 
% \caption{\small Comparisons of CCA algorithms in terms of the objective value Eq.~\eqref{eq:genrrr2}, as a function of iteration (top) and CPU runtime (bottom). Average $\pm$ standard deviation over 4 runs of the experiment.}\label{fig:cca_comparison} 
% \vspace{-5pt}
% \end{figure}

For further details on the RRMSE and CCA experiments, including the choice of hyperparameters and plots of convergence of the RRR constraint see supplementary materials Sec.~\ref{app:exp_details}.

==> old-stuff/old-sections/intro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  Intro



% In contrast to early sensory processing, subsequent processing in the cortex (both the neocortex~\cite{Spruston2008,Larkum2013,sjostrom2006,golding2002,gambino2014sensory} and the hippocampus~\cite{bittner2015,bittner2017behavioral,GreinbergerMagee2020,hardie2009synaptic}) is guided by supervisory signals. In particular, in cortical pyramidal neurons, proximal dendrites receive and integrate feedforward inputs leading to the generation of action potentials (i.e., the output of the neuron). The distal dendrites of the apical tuft, in contrast, receive and integrate instructive signals resulting in local depolarization. When the local depolarization is large relative to inhibitory currents, this generates a calcium plateau which propagates throughout the entire neuron. If the calcium plateau coincides with feedforward input it strengthens corresponding proximal synapses, thereby providing an instructive signal in these circuits~\cite{golding2002,sjostrom2006,bittner2017behavioral,GreinbergerMagee2020}.

% To account for these observations, the following  supervised and self-supervised learning models are available.  A normative model of cortical computation based on the predictive coding framework has been developed, explaining observed receptive fields~\cite{rao1999,rao2005probabilistic}.  However, this model has not been mapped onto the recently observed physiology and anatomy of cortical microcircuits. Recently, ~\cite{Payeur2020} extended earlier suggestions~\cite{kording2001supervised, guergiuev2016deep} that error backpropagation can be multiplexed with feedforward computation by relying on burst-dependant plasticity facilitated by calcium plateau potentials in the apical dendrites of pyramidal neurons. While these models propose a possible biological implementation of backpropagation, they rely on numerical simulations and optimize only the synaptic weights while postulating the architecture and the activity dynamics. Empirical models of these cortical circuits based solely on experimental evidence have also been proposed~\cite{Milstein2020}. However, a fully normative study of supervised neural networks which can explain recently observed experimental properties of cortical circuits is lacking.

% To serve as a viable model of brain function, an algorithm must satisfy at least the following two criteria~\cite{pehlevan2019neuroscience}. First, because sensory inputs are streamed to the brain and require real-time processing, it must be modeled by an online learning algorithm. To satisfy this requirement, unlike standard offline formulations which output projection matrices,  at each time step the algorithm must compute the output from the input of that time step. The weight matrices must be represented in synaptic weights and updated at each time step. Second, a neural network implementation of such an algorithm must rely exclusively on local synaptic learning rules. Here, locality implies that the plasticity rules depend exclusively on the variables available to the biological synapse, i.e. the physicochemical activities of the pre- and post-synaptic neurons in the synaptic neighborhood. An example of local learning is Hebb’s rule where the change of synaptic weight is proportional to the correlation between the output activities of the pre- and post-synaptic neurons~\cite{Hebb}.

==> old-stuff/old-sections/problem_statement.tex <==

In this section we review the general problem of Reduced-Rank Regression~(RRR) and recount how it encompasses Canonical Correlation Analysis (CCA) and Reduced Rank (minimum) Mean Square Error (RRMSE) as special cases.

\paragraph{Notation.~} For positive integers $m,n$, let $\R^m$ denote $m$-dimensional Euclidean space, and let $\R^{m\times n}$ denote the set of $m\times n$ real-valued matrices equipped with the Frobenius norm $\|\cdot\|_F$. 
We use boldface lower-case letters (e.g., $\v$) to denote vectors and boldface upper-case letters (e.g., $\M$) to denote matrices.
Let $\I_m$ denote the $m\times m$ identity matrix.

Let $\{(\x_t,\y_t)\}_{t=1}^T$ be a sequence of pairs of data points with $\x_t\in\R^m,\;\y_t\in\R^n$.
We refer to $\x_t$ as the predictor variable and $\y_t$ as the response variable.
Define the data matrices $\X:=[\x_1,\dots,\x_T]\in\R^{m\times T}$ and $\Y:=[\y_1,\dots,\y_T]\in\R^{n\times T}$.
Let $\C_{xx}:=\tfrac1T\X\X^\top$, $\C_{yy}:=\tfrac1T\Y\Y^\top$, and $\C_{xy}:=\tfrac1T\X\Y^\top$ be the empirical covariance matrices.
Throughout this paper, we assume that $\X$ and $\Y$ are centered and full rank.

\paragraph{Problem formulation.~} 
The goal of RRR is to find a low rank projection matrix $\P\in\R^{n\times m}$ that minimizes the error between $\P\X$ and $\Y$. 
The low rank constraint in this regression objective results in smaller over-fitting to the data and leads to the extraction of predictor features that are most predictive of the response variables~\cite{rrr_book}.
We can formalize this as follows:
% Let $\C_{xy}:=\tfrac1T\X\Y^\top$ be the empirical covariance matrix.
% Consider the generalized regression problem
\begin{align}
\label{eq:genrrr}
    \argmin{{\bf P}\in\R^{n\times m}} \frac1T\big\lVert \Y-\P\X \big\rVert_\Sigma^2 \quad\text{subject to}\quad\text{rank}(\P)\le k,
\end{align}
where $k\le\min(m,n)$ determines the rank of the problem, $\Sig\in\R^{n\times n}$ is a positive definite matrix, and $\|\cdot\|_\Sigma$ is the $\Sig$-norm defined by $\|\A\|^2_\Sigma:=\tr\A^\top\Sig\A$ for $\A\in\R^{n\times T}$.
%$\big\lVert \Y-\P\X \big\rVert_\Sigma^2 $ is the $\Sig$-norm of $(\Y-\P\X)$ defined as
% \begin{equation*}
%     \big\lVert \Y-\P\X \big\rVert_\Sigma^2 := \tr(\Y-\P\X)^\top\Sig(\Y-\P\X).
% \end{equation*}
Intuitively, the $\Sig$-norm is a generalized norm which can take into account the noise statistics of the samples~\cite{mahalanobis}. 
Two common choices for $\Sig$ are $\Sig=\I_n$ and $\Sig=\C_{yy}^{-1}$. 
When $\Sig=\I_n$, the RRR problem reduces to minimizing the mean square error (MSE) with a low rank constraint. We refer to this objective as Reduced Rank (minimum) Mean Square Error (RRMSE)~\cite{rrr_book}.\footnote{Also referred to as reduced rank Wiener filter or simply reduced rank regression depending on field of study.} 
For $\Sig=\C_{yy}^{-1}$, the objective in Eq.~\eqref{eq:genrrr} is equivalent to Canonical Correlation Analysis (CCA)~(see Sec.~\ref{app:CCA_from_grrr} of the supplementary materials).
% For a more detailed discussion of the relationship of CCA with the reduced rank regression task and intuitive interpretation see Sec.~\ref{app:CCA_from_grrr} of the supplementary materials.
% with $\Sig\in\R^{n\times n}$ a positive definite matrix (see e.g. \cite[Chapter 2.1]{rrr_book}).
% which defines the optimization norm

%  that normalizes the error between $\Y$ and $\P\X$. 
% The objective function in Eq.~\eqref{eq:genrrr} is closely related to many popular dimensionality reduction techniques in statistics \cite{izenman1975reduced}.
% For example:
% \begin{itemize}
%     \item When $\Y=\X$ and $\Sig=\I_n$, then this is an objective function for PCA.
%     \item When $\Sig=\I_n$ and $\P$ is full rank, this is usual linear regression.
%     \item When $\Sig=\C_{yy}$, this is CCA.
% \end{itemize}
 %for the historical background of the objective function in Eq.~\eqref{eq:genrrr}.

The low-rank constraint, $\text{rank}(\P)\le k$, in \eqref{eq:genrrr} can be enforced by expressing $\P=\Sig^{-1}\V_y\V_x^\top$, where $\V_x\in\R^{m\times k}$ and $\V_y\in\R^{n\times k}$ (the inclusion of $\Sig^{-1}$ here is for convenience in the derivation below).
The matrix $\V_x^\top$ projects the inputs $\x_t$ onto a $k$-dimensional subspace and the column vectors of $\Sig^{-1}\V_y$ span the range of the projection matrix $\P$. 
Plugging into Eq.~\eqref{eq:genrrr} we have
\begin{align}
\label{eq:genrrr1}
    \min_{\V_x\in\R^{m\times k}}\min_{\V_y\in\R^{n\times k}} \frac1T\big\lVert \Y-\Sig^{-1}\V_y\V_x^\top\X \big\rVert_\Sigma^2. 
    % = \Tr(\Y-\Sig^{-1}\V_y\V_x^\top\X)^\top\Sig^{-1}(\Y-\Sig\V_y\V_x^\top\X).
\end{align}
The minimum of this objective is not unique: given a solution $(\V_x,\V_y)$, for any invertible matrix $\M\in\R^{k\times k}$, $(\V_x\M^\top,\V_y\M^{-1})$ is also a solution. 
To constrain the solution set, we impose the whitening constraint $\V_x^\top\C_{xx}\V_x=\I_k$.
Expanding the quadratic in \eqref{eq:genrrr1}, dropping terms that do not depend on $\V_x$ or $\V_y$, and using the whitening constraint, we arrive at
% the following optimization problem:
\begin{align}\label{eq:genrrr2}
    \min_{\V_x\in\R^{m\times k}}\min_{\V_y\in\R^{n\times k}}\Tr(\V_y^\top\Sig^{-1}\V_y-2\V_x^\top\C_{xy}\V_y)\quad\text{subject to}\quad\V_x^\top\C_{xx}\V_x=\I_k.
\end{align}
% This objective function will be used for the derivation of our algorithms in the following section. 
The output of our algorithms will be the low rank projection of $\X$ which we call $\Z:=\V_x^\top \X$. Intuitively, for RRMSE ($\Sig = \I_n$), optimization of this objective would find $\Z$ which is most informative, in terms of MSE loss, of the response variable $\Y$. 
For CCA ($\Sig = \C_{yy}^{-1}$), optimization of this objective finds the projection $\Z$ which has the highest correlation with the response variable $\Y$. 

We parametrize the normalizing matrix by its inverse as $\Sig^{-1} = \Sig_s^{-1}:= s\,\C_{yy}  + (1-s)\, \I_n$ with $0\leq s \leq 1$. 
RRR with this normalizing matrix corresponds to a family of objectives which interpolate between RRMSE at $s=0$ and CCA at $s=1$.


% The linear RRR problem was introduced in \cite{}.

% When $\Y=\X$ and $\Sig=\I$, then the objective \eqref{eq:genrrr2} is PCA and $\V_x\x_t$ is the PCA projection with output whitening.
% Therefore, this can be viewed as a supervised PCA objective function.
% (Actually, this is exactly supervised PCA if we assume $\V_x^\top\V_x=\I_k$. Thus, we can view this as supervised PCA with output whitening.)
% When $\Sig=\C_{yy}$, the objective is related to CCA and $\V_x\x_t$ is the CCA projection for $\x_t$.

% In this work we focus on 2 cases: $\Sig=\I_n$ and $\Sig=\C_{yy}$.
% When $\Sig=\I_n$, the problem is referred to as FILL IN.
% When $\Sig=\C_{yy}$ the problem is related to CCA \cite{izenman1975reduced}.
% In fact, in this case, the projection $\V_x^\top\x_t$ is equal to the CCA projection (see Supplemental Material).

% \paragraph{Reduced Rank Regression.~} Reduced rank regression (RRR)~\cite{anderson1951estimating,izenman1975reduced}, is a variation of multi-variate linear regression where the matrix of regression weights is constrained to be low rank. 
% Explicitly, given centered predictor and response matrices $\X$ and $\Y$, RRR is formulated as minimizing the following objective  function:
% \begin{equation}\label{eq:rrr}
%     \min_{{\bf P}\in\R^{n\times m}} \big\big\lVert\Y - {\bf P} \X \big\big\rVert^2\quad\text{subject to}\quad\text{rank}({\bf P})\le k,
% \end{equation}
% where $\P\in\R^{n\times m}$ is the matrix of regression weights and $k\le\min(m,n)$ determines the rank of the problem. This low rank constraint can be explicitly implemented by letting $\P=\V_y \V_x^\top$ and rewriting the objective as
% \begin{equation}\label{eq:rrr_VxVy}
%     \min_{\V_x\in\R^{m\times k}}\min_{\V_y\in\R^{n\times k}} \big\big\lVert\Y - \V_y\V_x^\top \X \big\big\rVert^2.
% \end{equation}
% For any given solution to this optimization objective  $(\V_x,\V_y)$, there exists a family of solutions generated by invertible matrices $\M\in\R^{k\times k}$ given by $(\V_x\M^\top,\V_y\M^{-1})$.
% It is common to reduce this degeneracy of solutions by imposing the whitening constraint $\V_x^\top \C_{xx} \V_x=\I_k$. 
% Expanding the quadratic in \eqref{eq:rrr_VxVy}, ignoring the constant $\Y\Y^\top$ term, and using the whitening constraint, we arrive at the following objective:
% \begin{equation}\label{eq:RRR_first}
%     \min_{\V_x\in\R^{m\times k}}\min_{\V_y\in\R^{n\times k}}\tr\V_y^\top\V_y-2\V_x^\top \C_{xy}\V_y,\quad\text{subject to}\;\V_x^\top \C_{xx}\V_x=\I_k.
% \end{equation}
% Reduced rank regression has wide applications~\cite{rrr_book}. This is in part because it can be used as an explicit regularizer to reduce over-fitting of the responses~\cite{izenman1975reduced}. But also because it is an effective tool for dimensionality reduction~\cite{sparese_rrr} in the sense that the projection matrix $\V_x^\top \X$ is the subspace of the predictor matrix $\X$ which is maximally informative of the responses $\Y$. In this interpretation, RRR is not an algorithm for inferring the response of a system, but much like canonical correlation analysis, it is a self-supervised  algorithm where part of the data is being used to compress the rest. 

% \paragraph{Canonical correlation analysis.~} Introduced by Hotelling in 1936~\cite{hotelling1936relations}, canonical correlation analysis is a statistical tool for dimensionality reduction based on the cross-correlation of two multi-dimensional variables~\cite{cca_tutorial}.  Explicitly, given two data matrices $\X$ and $\Y$, the CCA objective is to find the subspace of $\X$ and $\Y$ such that their cross-correlation is maximized:
% \begin{align}\label{eq:CCA_lin_obj}
%     \argmax{\W_x\in\R^{m\times k},\W_y\in\R^{n\times k}}\tr\left(\W_x^\top \C_{xy}\W_y\right) ,\quad\text{subject to}\;
%     \W_x^\top\C_{xx}\W_x=\W_y^\top \C_{yy}\W_y=\I_k.
% \end{align}
% To proceed, it is convenient to use the eigenvalue formulation of CCA~(see Sec.~\ref{app:CCA_op_2_eig} of supplementary materials):
% \begin{align}\label{eq:CCA_eig_start}
%     \C_{xx}^{-1}\C_{xy}\C_{yy}^{-1}\C_{yx}\V_x=\V_x\Lam^2,\quad\text{subject to}\;\V_x^\top\C_{xx}\V_x=\I_k,
% \end{align}
% where $\Lam$ is the diagonal matrix of canonical correlations\footnote{\note{SG: this is only diagonal in the correct basis and the derivation in the appendix does not necessarily bring it into this diagonal form.}} and columns of $\V_x$ are the canonical correlation basis vectors. Multiplying on both sides by $\V_x^\top\C_{xx}$ we arrive at
% \begin{align*}
%     \V_x^\top\C_{xy}\C_{yy}^{-1}\C_{yx}\V_x=\Lam^2,
% \end{align*}
% where we have used the constraint $\V_x^\top\C_{xx}\V_x=\I_k$. We can therefore find the subspace spanned by the canonical basis elements corresponding to the highest eigenvalues as the span of the columns of the matrix $\V_x$ which maximizes the following objective.
% \begin{equation}
%     \max_{\V_x\in\R^{m\times k}} \tr\V_x^\top\C_{xy}^\top \C_{yy}^{-1}\C_{yx}\V_x,\quad\text{subject to}\;\V_x^\top \C_{xx}\V_x=\I_k.
% \end{equation}
% We can simplify this objective by introducing an auxiliary variable $\V_y$. Multiplying by an overall minus sign and switching from $\max$ to $\min$ brings us to
% \begin{equation}\label{eq:CCA_first}
%     \min_{\V_x\in\R^{m\times k}}\min_{\V_y\in\R^{n\times k}}\tr\V_y^\top\C_{yy}\V_y-2\V_x^\top\C_{xy}\V_y,\quad\text{subject to}\;\V_x^\top\C_{xx}^\top\V_x=\I_k.
% \end{equation}
% In this formulation the matrix $\V_x$ is the same as the $\W_x$ matrix in the formulation of Eq.~\eqref{eq:CCA_lin_obj}. However, while $\V_y$ and $\W_y$ span the same subspace, $\V_y$ does not satisfy the same normalization constraint, i.e. $\W_y = (\V_y^\top \C_{yy}\V_y)^{-1/2} \V_y$. For more details see supplementary materials Sec.~\ref{app:CCA_op_2_eig}.

% Comparison of the RRR and CCA objective in Eqs.~\eqref{eq:RRR_first} and ~\eqref{eq:CCA_first} demonstrates the close relationship between the two methods~\cite{cca_tutorial,rrr_book,de2012least}. In the following sections we show how these objectives can be turned into online algorithms and then into biologically plausible neural networks. 
% The derivation of the algorithm for each problem is similar, however, for clarity we will consider them separately.

==> old-stuff/old-sections/rrr.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%% RRR algorithm %%%%%%%%%%%%%%%%%%%%%%%%

% In this section, we derive the biologically plausible algorithm for reduced rank regression starting from the objective function in Eq.~\eqref{eq:RRR_first}
% \begin{equation*}
%     \min_{\V_x\in\R^{m\times k}}\min_{\V_y\in\R^{n\times k}}\tr\V_y^\top\V_y-2\V_x^\top\C_{xy}\V_y,\quad\text{subject to}\;\V_x^\top\C_{xx}\V_x=\I_k.
% \end{equation*}
% Noting that imposing the constraint $\V_x^\top\C_{xx}\V_x=\I_k$ via a Lagrange multiplier (as in Sec.~\ref{app:CCA_op_2_eig}) leads to non-local update rules for the weight matrices, following \cite{pehlevan2015normative} we instead  impose the weaker inequality constraint $\V_x^\top\C_{xx}\V_x  \preceq \I_k$ by introducing the matrix $\Q\in\R^{k \times k}$
% \begin{equation}\label{eq:rrr_final}
%     \min_{\V_x\in\R^{m\times k}}\min_{\V_y\in\R^{n\times k}}\max_{\Q\in\R^{k \times k}} \tr\V_y^\top\V_y-2\V_x^\top\C_{xy}\V_y+\Q\Q^\top(\V_x^\top\C_{xx}\V_x-\I_k),
% \end{equation}
% where $\Q\Q^\top$ is the positive semi-definite Lagrange multiplier enforcing the inequality. Just as in \cite{pehlevan2015normative}, the dynamics of the optimization then enforce that the inequality constraint is saturated (for a different proof see Sec.~\ref{app:rrr_sol_details}). This objective can be optimized using gradient descent-ascent dynamics derived by taking partial derivatives:
% \begin{align}\label{eq:rrr_offline_updates}
%     \V_x^\top&\gets\V_x^\top+\eta(\V_y^\top \C_{yx}-\Q\Q^\top\V_x^\top\C_{xx})\notag\\
%     \V_y^\top&\gets\V_y^\top+\eta(\V_x^\top \C_{xy}-\V_y^\top)\\
%     \Q&\gets\Q+\frac{\eta}{\tau}(\V_x^\top\C_{xx}\V_x-\I_k)\Q,\notag
% \end{align}
% where $\eta>0$ is the learning rate for $\V_x$ and $\V_y$, and $\tau>0$ is a parameter controling the ratio of the descent and ascent steps.

% \paragraph{Online algorithm.}~

% The online RRR algorithm is derived from the objective function~\eqref{eq:rrr_final} using stochastic gradient descent-ascent, i.e. by taking gradient steps of the objective function computed on one sample at a time. To simplify notation and make biological plausibility manifest, we define $\Z$ as the projected predictor data matrix $\Z:=\V_x^\top \X$ respresenting the output neurons of the network, and introduce neural variable $\N := \Q^\top \Z$ representing a set of interneurons connected to the output neurons~$\Z$ via the synaptic weight matrix~$\Q^\top$. 

% The online update rule at time $t$ when presented by inputs $\x_t$ and $\y_t$ is then given by
% \begin{align}\label{eq:rrr_online_updates}
%     \V_x^\top&\gets\V_x^\top+\eta(\V_y^\top \y_t-\Q\n_t)\x_t^\top\notag\\
%     \V_y^\top&\gets\V_y^\top+\eta(\z_t\y_t^\top-\V_y^\top)\\
%     \Q&\gets\Q+\frac{\eta}{\tau}(\z_t\n_t^\top-\Q).\notag
% \end{align}
% We leave the biological interpretation of this algorithm to Sec.~\ref{sec:circuit}. Here we just note that the algorithm is local in that the update rule for any synapse $S_{ij}$ connecting neurons $i$ and $j$ only depends on itselfand on the synaptic weight modulated activty of adjacent neurons (e.g. $\V_y^\top \y_t$ or $\Q\n$) which are all locally available to the neuron.

